PathE: Leveraging Entity-Agnostic Paths for Parameter-Efficient Knowledge Graph Embeddings

Knowledge Graphs (KGs) store human knowledge in the form of entities (nodes) and relations, and are used extensively in various applications. KG embeddings are an effective approach to addressing tasks like knowledge discovery, link prediction, and reasoning. This is often done by allocating and learning embedding tables for all or a subset of the entities. As this scales linearly with the number of entities, learning embedding models in real-world KGs with millions of nodes can be computationally intractable. To address this scalability problem, our model, PathE, only allocates embedding tables for relations (which are typically orders of magnitude fewer than the entities) and requires less than 25% of the parameters of previous parameter efficient methods. Rather than storing entity embeddings, we learn to compute them by leveraging multiple entity-relation paths to contextualise individual entities within triples. Evaluated on four benchmarks, PathE achieves state-of-the-art performance in relation prediction, and remains competitive in link prediction on path-rich KGs while training on consumer-grade hardware. We perform ablation experiments to test our design choices and analyse the sensitivity of the model to key hyper-parameters. PathE is efficient and cost-effective for relationally diverse and well-connected KGs commonly found in real-world applications.

==> notes.tex <==
\section{Tracing KG properties for effective representations}\label{sec:suitability}

\todo[inline]{See alternative version below}

The various benchmark datasets that are used for the evaluation of embedding models exhibit very diverse structural properties, both due to the nature of the source KG as well as due to the way the triples have been sampled to create the benchmark.
Moreover, we found that, following the training-validation-test split of these benchmark datasets, some triples may retain very little connectivity patterns such as cliques, connected components etc., of the original KG.
We expect this structurally-agnostic split of triples to inherently affects the ability of relation-based path-based methods (including PathE) to learn such patterns.

This diversity is reflected on measurements of the number and distribution of relations, the number of unique relational contexts of nodes and the number and uniqueness of the paths mined from each dataset.
Specifically, as seen in Table~\ref{tab:dataset-stats}, the number of unique relations varies significantly between the datasets with the smaller number being 11 for WN18RR and the largest being 237 for FB15K-237.
This has been demonstrated to have a significant impact on inductive models that only use relations to encode both the relations and entities as it significantly limits their ability to discriminate between entities \cite{nodepiece}.

% To address this problem and make discriminating between nodes easier, PathE also utilises the frequency of relations in the relational contexts of each entity, which allows relations that appear multiple times in the context of the entity to be represented by their count instead of a binary encoding (1 or 0).
% It is evident that this encoding scheme works effectively as the entity degree becomes higher and the ratio of the relation types in the KG is not too unbalanced.

As shown in Section~\ref{ssec:link-prediction}, despite its parameter efficiency, inherent inductive bias and its state-of-the-art performance on all benchmark datasets when compared to Nodepiece without anchors, our model performs worse on WN18RR and YAGO3-10 compared to FB15k-237 and CoDEx-Large.
As such, it is of central importance to determine what are the characteristics of the datasets that our model performs well at, so that researchers and practitioners can determine the applicability of the method prior to using resources for training a model.

Therefore, we sought to investigate the unique relational contexts of each dataset, which are used to encode the entities of the KG, and the ratios of the relations.
As seen in Table \ref{tab:edge-stats}, in WN18RR and YAGO3-10 the top two relations account for more than 74\% and 64\% of the total respectively, making these datasets extremely unbalanced.
This, coupled with their small number of relation types (11 and 36) and the average entity degree of 4.28 and 17.52, severely limits the informativeness of unique relational contexts (or unique entity encodings) that exist in the datasets.
In particular, the unique relational contexts of WN18RR are 3,264, which are used to encode 40,559 entities and for YAGO3-10 they are 24,500, used to encode 123,143 entities.
This produces a coverage of 0.080 and 0.198 of the entities respectively.

In comparison, as seen in Table \ref{tab:edge-stats-2}, FB15K-237 and CoDEx-Large have a much less unbalanced relation ratio, a larger number of unique relations (237 and 69) and large average entity degrees that amount to 37.5 for FB15K-237 and 14.14 for CoDEx-Large.
This brings the unique relational contexts to 13,352 for FB15K-237 and  36,202 for CoDEx-Large, covering 0.920 and 0.464 of the entities, respectively.

In conclusion, by relating the number of unique relations, average entity degree, and the uniqueness of relational contexts on which paths are defined, we observe that there is a clear trend for the applicability of PathE in link prediction.
One such example is the largest open-source KG, Wikidata, which has 12353 unique relations (called properties), more than 115 million entities (items) and contains in excess of 1.6 billion statements to date\footnotemark[1].
Based on its rich relational dictionary, its somewhat balanced distribution of relations shown in Table~\ref{tab:edge-stats-3} and its average node degree of 29, it is apparent that Wikidata exhibits similar characteristics to FB15k-237 and CoDEx-Large.
In addition, its very large size makes the application of any embedding method which uses the entire adjacency matrix, such as CompGCN \cite{compgcn}, NeuralLP \cite{NeuralLP} and DRUM \cite{DRUM} intractable due to the required memory size.
Furthermore, its dynamic nature with additions of nodes happening daily, makes it challenging to apply traditional KGE methods that store full embedding tables, such as RotatE \cite{Rotate}, TransE \cite{TransE} and ConvE \cite{ConvE}.
% \todo[inline]{Not sure about this)}
% Moreover, assuming a configuration similar to the one used for FB15k-237, with embeddings of dimension 200 and less than 10\% of the total nodes encoded as suggested in \cite{nodepiece}, a Nodepiece model would require approximately $2*10^9$ parameters for the anchors plus $2.4*10^6$  parameters for encoding the relations, whereas a PathE model of configuration similar to the one reported in this paper would require less than $10^6$ parameters.

In sum, for datasets showing a rich relational vocabulary with path-rich relational contexts, such as FB15K-237 and CoDEx-Large, PathE provides a competitive solution compared to current parameter-efficient methods.
However, for KGs showing limited relational vocabulary and low diversity (class imbalance), we advocate for the use of other parameter-efficient methods, such as Nodepiece and EARL -- where the use of anchors or reserved entities provides the best link prediction performance.

% % Appendix D: Analysis of Knowledge Graph Properties and Their Influence on PathE Performance

% \section{Analysis of KGs Properties and their influence on PathE performance}

% PathE relies on encoding entities based on their relational contexts and the paths traversing those relations.
% %
% The richness and diversity of these contexts are thus central for generating discriminative entity representations.
% %
% This section examines the relationship between the structural characteristics of KGs and the efficacy of PathE for link prediction.
% %
% The experiments detailed in Section~\ref{sec:experiments}, demonstrate that PathE performs well on FB15k-237 and CoDEx-Large, but yields less competitive results on WN18RR and YAGO3-10.
% %
% We posit that these performance discrepancies are primarily attributable to variations in relational diversity, entity degree, and the uniqueness of relational contexts across these datasets.

% \begin{enumerate}
%     \item \textbf{Relational Diversity}.
%     A greater number of distinct relation types provides a more expressive vocabulary for characterising entities and their interconnections.    
%     This potentially facilitate the model to capture more nuanced relationships and distinguish between entities with greater accuracy.

%     \item \textbf{Average Entity Degree}.
%     A higher average degree generally signifies a denser graph with more connections per entity.
%     This translates to a greater number of paths traversing each entity, providing the model with more contextual information for embedding entities.

%     \item \textbf{Uniqueness of Relational Contexts}.
%     The extent to which entities can be uniquely identified based solely on their relational contexts is also central.
%     A higher proportion of unique contexts indicates that the relational structure provides strong discriminatory signals for differentiating between entities.
% \end{enumerate}

% Tables \ref{tab:dataset-stats}, 11 and 12 provide insights into the structural differences between the benchmark datasets.
% We analyse these differences in relation to PathE's performance.

% \begin{itemize}
%     \item \textbf{WN18RR and YAGO3-10 (sparse KGs).}
%     These datasets are characterised by limited relational diversity, possessing only 11 and 37 distinct relation types, respectively.
%     %
%     Furthermore, they exhibit a highly skewed distribution of relations.
%     %
%     In WN18RR, the two most frequent relations account for over 74\% of all triples, while in YAGO3-10, they constitute over 64\%.
%     %
%     This combination of limited relational diversity, low average entity degree, and a paucity of unique relational contexts (8\% for WN18RR and 19.8\% for YAGO3-10) significantly hinders PathE's ability to learn discriminative entity embeddings.
%     %
%     The relational contexts are simply too homogeneous to effectively distinguish between entities.
%     %
%     The results of the inductive experiments, where PathE performs poorly on WN18RR V1, V2 and V4 further corroborate this observation.
%     %
%     These particular datasets have the lowest number of unique relations (9,10 and 9 respectively), which constrains the model's capacity to learn the underlying semantics of the relations.

%     \item \textbf{FB15k-237 and CoDEx-Large (path-rich KGs).}
%     In contrast, these KGs exhibit considerably higher relational diversity, with 237 and 69 distinct relation types, respectively, and a more balanced distribution of relations.
%     Their higher average entity degrees (37.5 and 14.14) and, crucially, a much larger proportion of unique relational contexts (92\% for FB15k-237 and 46.4\% for CoDEx-Large) provide PathE with a significantly richer set of features from which to learn.
%     %
%     These factors enable the model to effectively capture the diverse relationships and generate more discriminative entity representations, resulting in superior link prediction performance.
%     %
%     % The inductive experiments, where PathE outperforms other path-based methods on FB15K-237 V1 and V2, further support this claim, as these versions possess a higher number of unique relations compared to the similarly structured V5 (117, 129, and 101 respectively).
%     The inductive experiments, where PathE outperforms other path-based methods on FB15K-237 V1 and V2 and even matches the performance of the best performing method on V1, further support this claim.
% \end{itemize}

% This analysis underscores that PathE performs better in KGs characterised by high relational diversity, rich relational contexts, and high uniqueness of relational contexts.
% %
% These characteristics are frequently observed in large, real-world KGs.
% %
% For instance, Wikidata counts 12353 unique relations (called properties), more than 115 million entities (items) and contains 1.6+ billion statements to date\footnotemark[1].
% As reported in Table~\ref{tab:edge-stats-3}, Wikidata has a balanced distribution of relations and an average node degree of 29.
% %
% % These properties, coupled with the inherent intractability of methods relying on the full adjacency matrix for a KG of this scale, suggest that PathE is potentially well-suited for application to Wikidata and KGs exhibiting similar structural features.
% While more experiments are needed to assess PathE's applicability to Wikidata, here we remark that these characteristics are better represented by the FB15k-237 and CoDEx-Large benchmarks, which are indeed derived from Freebase and Wikidata, respectively.

% % Overall, we emphasise that the efficacy of PathE is linked to the structural characteristics of the underlying KG.
% %
% In conclusion, while parameter-efficient methods such as NodePiece \cite{nodepiece} and EARL \cite{EARL}, which depend on anchors or reserved entities, are preferable for KGs with limited relational diversity and low uniqueness of relational contexts, PathE emerges as a highly competitive and scalable solution for large, densely connected KGs with diverse relational vocabularies.
% This is especially relevant when a lightweight model is required for link prediction.
% Nonetheless, and irrespective of the efficiency requirements, PathE achieves state-of-the-art performance in relation prediction, surpassing other parameter-efficient methods and making it a particularly compelling choice when relation prediction is the primary objective.
